A Framework for Reproducible Benchmarking and Performance Diagnosis of SLAM Systems

We propose SLAMFuse, an open-source SLAM benchmarking framework that provides consistent crossplatform environments for evaluating multi-modal SLAM algorithms, along with tools for data fuzzing, failure detection, and diagnosis across different datasets. Our framework introduces a fuzzing mechanism to test the resilience of SLAM algorithms against dataset perturbations. This enables the assessment of pose estimation accuracy under varying conditions and identifies critical perturbation thresholds. SLAMFuse improves diagnostics with failure detection and analysis tools, examining algorithm behaviour against dataset characteristics. SLAMFuse uses Docker to ensure reproducible testing conditions across diverse datasets and systems by streamlining dependency management. Emphasizing the importance of reproducibility and introducing advanced tools for algorithm evaluation and performance diagnosis, our work sets a new precedent for reliable benchmarking of SLAM systems. We provide ready-to-use docker compatible versions of the algorithms and datasets used in the experiments, together with guidelines for integrating and benchmarking new algorithms. Code is available at https://github.com/nikolaradulov/slamfuse

==> figures/brightness.tex <==
% \begin{figure}[hb]
%   \centering
%   \includegraphics[width=\linewidth]{images/brightness_orbslam3_kitti.png}
%   \caption{General shape of algorithm breakpoints with regards to shaprness, exemplified by orbslam3 on KITTI07}
%   \label{fig:orb3_brightness}
% \end{figure}

==> figures/contrast_orbslam3.tex <==



% \begin{figure}
%     \centering
%     \begin{subfigure}[a]{0.49\linewidth}
%         \includegraphics[width=\linewidth]{images/brightness_orbslam3_tum.png}
%         \caption{Brightness effect on orbslam3, freiburg1 desk1 trajectory}
%     \end{subfigure}
%     \begin{subfigure}[a]{0.49\linewidth}
%         \includegraphics[width=\linewidth]{images/brightness_lsdslam_tum.png}
%         \caption{Brightness effect on lsdslam, freiburg1 desk1 trajectory}
%     \end{subfigure}
%     \\
%     \begin{subfigure}[a]{0.49\linewidth}
%         \includegraphics[width=\linewidth]{images/brightness_orbslam3_tum1.png}
%         \caption{Brightness effect on orbslam3, freiburg1 xyz and rpy trajectories}
%     \end{subfigure}
%     \begin{subfigure}[a]{0.49\linewidth}
%         \includegraphics[width=\linewidth]{images/lsd_xyz_brightness.png}
%         \caption{Brightness effect on lsdslam, freiburg1 xyz and rpy trajectories}
%     \end{subfigure}
%     \caption{}
%     \label{fig:grid}
% \end{figure}


\begin{figure}[!htb]
    \centering

   
    
    % --- Subfigure b ---
    \begin{subfigure}[b]{\columnwidth}
        \includegraphics[width=\linewidth]{images/contrast_orbslam3_tum1.png}
        \label{Figure:darpa images metrics}
    \end{subfigure}
     \vspace{1ex} % Space between subfigures
    % --- Subfigure a ---
    \begin{subfigure}[a]{\columnwidth}
        % Top Left Image
        \begin{minipage}[a]{0.49\linewidth}
            \includegraphics[width=\linewidth]{images/contrast_orbslam3_kitti.png}
        \end{minipage}
        \hfill
        % Top Right Image
        \begin{minipage}[a]{0.49\linewidth}
            \includegraphics[width=\linewidth]{images/contrast_orbslam3_tum.png}
        \end{minipage}
        \label{Figure:orbslam3 contrast}
    \end{subfigure}

    
    \caption{Influence of contrast of Orbslam3 breakpoints}
    \label{Figure:orbslam3_contrast}
\end{figure}

==> figures/fuzzing_brightness.tex <==
\begin{figure}
  \centering
  \includegraphics[width=\linewidth]{images/brightness_orbslam3_kitti.png}
  \caption{General shape of algorithm breakpoints with regards to shaprness, exemplified by orbslam3 on KITTI07}
  \label{fig:orb3_brightness}
\end{figure}

\begin{figure}
    \centering
    \begin{subfigure}[a]{0.49\linewidth}
        \includegraphics[width=\linewidth]{images/brightness_orbslam3_tum.png}
        \caption{Brightness effect on orbslam3, freiburg1 desk1 trajectory}
    \end{subfigure}
    \begin{subfigure}[a]{0.49\linewidth}
        \includegraphics[width=\linewidth]{images/brightness_lsdslam_tum.png}
        \caption{Brightness effect on lsdslam, freiburg1 desk1 trajectory}
    \end{subfigure}
    \\
    \begin{subfigure}[a]{0.49\linewidth}
        \includegraphics[width=\linewidth]{images/brightness_orbslam3_tum1.png}
        \caption{Brightness effect on orbslam3, freiburg1 xyz and rpy trajectories}
    \end{subfigure}
    \begin{subfigure}[a]{0.49\linewidth}
        \includegraphics[width=\linewidth]{images/lsd_xyz_brightness.png}
        \caption{Brightness effect on lsdslam, freiburg1 xyz and rpy trajectories}
    \end{subfigure}
    \caption{}
    \label{fig:grid}
\end{figure}


==> figures/legoloam.tex <==
\begin{figure}[!tb]
    \centering
    \begin{minipage}{0.49\linewidth} % Adjust width as needed
        \includegraphics[width=\linewidth, height=0.65\linewidth]{images/legoloam_kitti.JPG}
    \end{minipage}
    \begin{minipage}{0.49\linewidth} % Adjust width as needed
        \includegraphics[width=\linewidth, height=0.65\linewidth]{images/legoloam_newer.JPG}
    \end{minipage}
    \caption{Visualized execution results of LeGO-LOAM running on KITTI Dataset (left) and Newer College Dataset (right) in SLAMBench4.}
    \label{fig:legoloam_on_dataset}
\end{figure}

==> figures/legoloam_visualization.tex <==
\begin{figure}[tb!!]
    \centering
    \begin{minipage}{0.49\linewidth}
    \fbox{\includegraphics[width=\dimexpr\linewidth-2\fboxrule-2\fboxsep\relax, height=0.55\linewidth]{images/legoloam_kitti01_corn.png}}
    \end{minipage}
    \hfill
    \begin{minipage}{0.49\linewidth}
        \fbox{\includegraphics[width=\dimexpr\linewidth-2\fboxrule-2\fboxsep\relax, height=0.55\linewidth]{images/legoloam_kitti07_corn.png}}
    \end{minipage}
    \caption{Comparison of extracted edge features (blue) by LeGO-LOAM on KITTI sequence 01 (left) and sequence 07 (right). Note the effects on error observed in Figure \ref{Figure:kitti_ate_rmse}}
    \label{Figure:legoloam_edge_points}
\end{figure}

